A Pre-Trained Graph-Based Model for Adaptive Sequencing of Educational Documents

Massive Open Online Courses (MOOCs) have greatly contributed to making education more accessible. However, many MOOCs maintain a rigid, one-size-fits-all structure that fails to address the diverse needs and backgrounds of individual learners. Learning path personalization aims to address this limitation, by tailoring sequences of educational content to optimize individual student learning outcomes. Existing approaches, however, often require either massive student interaction data or extensive expert annotation, limiting their broad application. In this study, we introduce a novel data-efficient framework for learning path personalization that operates without expert annotation. Our method employs a flexible recommender system pre-trained with reinforcement learning on a dataset of raw course materials. Through experiments on semi-synthetic data, we show that this pre-training stage substantially improves data-efficiency in a range of adaptive learning scenarios featuring new educational materials. This opens up new perspectives for the design of foundation models for adaptive learning.

==> abstract.tex <==
Learning path personalization is a critical challenge in the realm of adaptive learning and educational technology.
It aims to tailor a sequence of educational activities to optimize individual student learning outcomes.
Reinforcement learning (RL) has long been identified as a promising approach to address this problem, however low sample efficiency hinders its application to real-world scenarios.
In this paper, we present an approach to improve sample efficiency on this task using transfer learning.
First, we introduce a set of readily available source tasks that are close but different from the target task of learning path personalization.
Then we show that pre-training an RL agent on these source tasks increases the sample efficiency on the target adaptive learning task, opening new perspectives for efficient implementations of RL algorithms in personalized learning environments.
